Evaluating Feedback-Driven Black-Box Processes via Stochastic Modeling and Simulation

We study feedback-driven black-box processes across software engineering and machine learning. These processes are inherently sequential: policies generate inputs, observe outputs/feedback from systems, and use the feedback to guide the design of subsequent inputs. While many policies are developed under structural assumptions on the underlying systems, many real-world systems operate without such knowledge, necessitating black-box policies that lack a unified evaluation framework. We introduce a stochastic framework that models and evaluates such policies using Markov chains and simulation, thereby connecting empirical practice with theory. We instantiate the framework in mutation-based fuzzing (widely used for discovering software bugs via sequential input mutation), by a novel Markov chain model of fuzzing whose transitions are governed by the mutation strategy and whose feedback is given by program execution. We develop a rigorous evaluation paradigm with new performance measures, sound estimators, and evaluation procedures with provable guarantees. Guided by the theory, we evaluate 9 fuzzers on 18 widely used fuzzing benchmarks and conduct case studies in 4 non-fuzzing domains. These results show that the framework provides a principled basis for evaluation while connecting to practice, with implications beyond fuzzing.

==> sections/abstract.tex <==
\begin{abstract}
Fuzzing, especially mutation-based fuzzing, is widely used to identify vulnerabilities (i.e., bugs) in software programs by generating input strings with fuzzers and feeding them to the target program. The goal of a fuzzing technique (fuzzer) is to uncover as many bugs as possible by mutating existing inputs. Numerous fuzzing techniques have been proposed and shown to be effective via empirical evaluations, yet the underlying fuzzing process remains poorly understood in terms of its inherent randomness, and no unified objective exists to represent this goal. Importantly, fuzzer performance is typically assessed by experiments, where metrics are computed after running the fuzzing process for a fixed duration, without theoretical guarantees to guide rigorous evaluation. There have also been ongoing debates over these metrics, as each has its own merit and concerns. These limitations may hinder the generalizability of fuzzers across domains, at the risk of inconsistent performance on different software.

To this end, we present the first rigorous framework for understanding and evaluating the fuzzing process via stochastic modeling and simulation. Specifically, we model the fuzzing process as a Markov chain, where the state space corresponds to the program’s input space, and each mutation represents a transition in this space, with a transition probability matrix determined by the fuzzer. The feedback we observe is a function of this process, with a two-dimensional state space (bug/no bug), which allows us to define a unified objective. Building on this foundation, we propose an evaluation framework grounded in both theory and practice. We define a performance measure, design methods to construct an estimator, and establish evaluation metrics based on the proven statistical properties of the estimator. This framework further enables the derivation of practical yet rigorous guidelines for evaluating and designing fuzzers. Finally, we comprehensively evaluate nine fuzzers on 18 popular benchmarks, showing that the empirical results validate the theoretical effectiveness. We also propose general guidelines that unify, refine, and extend existing practices while informing future fuzzer designs.
\end{abstract}


==> sections/backup.tex <==
input-output aligned; general operations/processes

black-box aligned process

partially black-box

hybrid; close-loop; adaptive black-box, 

feedback-driven black-box  process solved by markov chains; black-box process 

machine learning problems that can be modeled as feedback-driven black-box processes 

CMAES; generic algorithm; genetic ; parameter tuning systems (combinatorial optimization; random mutation, heuristics, rules, feedback driven); -> several sentences 

fuzzing (specific, more elaborations) -> evaluation on fuzzing; 


dynamic pricing/advertisement bidding/reinforcement learning -> one sentence 


related work: black-box processes, genetic, tuning systems, 

$x_0 -> g(x_0)$
$x_1, x_2 -> g, $ inference $g$; design points $x$ maximize $g$, sequential dependency, adaptive

$x_0 -> (f(x_0), f_1(x_0))= 1_{x_0 \in B},  -> x_1 = g(f, x_0) -> f(x_1) -> x_2 = g(f, x_1)$ (hidden markovian model)


1. Traditional Black-Box System

Definition

A traditional black-box system is modeled as a static input–output mapping:

g : \mathcal{X} \rightarrow \mathcal{Y}

where:
	•	\mathcal{X} is the input space,
	•	\mathcal{Y} is the output (observation) space,
	•	g is unknown but fixed.

Execution

Given an input x \in \mathcal{X}, the system produces:

y = g(x)

Key Properties
	1.	No state
g(x) \text{ is independent of past inputs or outputs}
	2.	No adaptation
x \text{ is chosen independently of } y
	3.	One-shot interaction
(x, y) \text{ pairs are i.i.d. samples}

Interpretation

This model captures:
	•	Classical black-box testing
	•	Random testing
	•	Property-based testing without feedback

⸻

2. Feedback-Driven Black-Box Process

Definition

A feedback-driven black-box process is a dynamical system formed by the composition of:

g : \mathcal{X} \rightarrow \mathcal{Y}
\quad\text{(system under test)}

f : \mathcal{Y} \times \mathcal{S} \rightarrow \mathcal{X} \times \mathcal{S}
\quad\text{(feedback / adaptation function)}

where:
	•	\mathcal{S} is an internal process state (e.g., corpus, coverage summary).

Execution

Initialize:
(x_0, s_0) \sim \mu_0

Iterate for t = 0, 1, 2, \dots:

y_t = g(x_t)

(x_{t+1}, s_{t+1}) = f(y_t, s_t)

Key Properties
	1.	Stateful
s_{t+1} = \phi(s_t, y_t)
	2.	Adaptive
x_{t+1} \sim P(\cdot \mid y_{\le t})
	3.	Sequential dependence
x_{t+1} \not\!\perp\!\!\!\perp x_t

Interpretation

This model captures:
	•	Coverage-guided fuzzing
	•	Evolutionary fuzzing
	•	Reinforcement-style test generation

⸻

3. Side-by-Side Mathematical Contrast

Aspect	Traditional Black-Box	Feedback-Driven Black-Box
Mapping	g(x)	f(g(x_t), s_t)
State	None	s_t
Time	Single-step	Multi-step
Input choice	Fixed / random	Feedback-dependent
Dependence	i.i.d.	Markovian or non-Markovian


⸻

4. Compact Formal Distinction

A traditional black-box system satisfies:

\forall t,\; x_t \sim \mu \quad\text{independently}

A feedback-driven black-box process satisfies:

x_{t+1} = F(g(x_t), \dots, g(x_0))

for some (possibly stochastic) functional F.

⸻

5. One-Line Summary (Paper-Ready)

A traditional black-box system is a static input–output mapping g, whereas a feedback-driven black-box process is a closed-loop dynamical system defined by the iterative composition x_{t+1} = f(g(x_t), s_t).

\clearpage 
\newpage 
\hl{***Discussions of the estimation of $\delta_R$***}

\hl{solution: can we compute this for each fuzzer based on the historical data; we have the following formula}

\(\delta_R = \frac{1}{\gamma_R} =  \leq (\frac{4}{\log{(\frac{2}{1 + 4\epsilon + 2\epsilon^2})}}) \tau(\epsilon)\) 
where \(\tau(\epsilon)\) is the mixing time defined as \(\min_{t}\lVert P_{R}^t(x,\cdot) - \pi \rVert_{TV} \leq \epsilon\).

\hl{mixing time can be approximated by the procedure in [38] or can we use the mixing time of the output process as the approximation?}



\hl{***mutation step and time alignment:***}

\hl{we can always set the total mutation steps to be the maximum number of mutations, and then we can say that for fuzzers that mutation less than that, the extra mutations steps are just not staying at the current positions in the input space}

% I got this from gpt, it seems reasonable to me: The idea here is to align fuzzers on a common step axis by taking the maximum number of mutations $N_{\max}$ observed (e.g., within a fixed wall-clock budget) and “padding” slower fuzzers with self-loops—i.e., treating the remaining steps as staying at the current state. This is mathematically valid as a bookkeeping device (it effectively makes the chain “lazy”), but it can be semantically misleading: a slower fuzzer is not idle—it is spending more time per step on generation/execution/analysis. Moreover, adding self-loops changes the effective transition kernel (and thus spectral/mixing properties), so one should be careful not to draw mechanistic conclusions from the padded process.


\hl{the mutation time is deterministic or random?}

% It's not deterministic, but it's also not totally random. The changes may be dependent on many factors, like mutation strategy itself, how this fuzzer is executed, the machine the fuzzer is running on itself(have different load, other threads occupying resources)

\hl{we build better fuzzers on top of AFL instead of injecting seed corpus or scheduling.}
% what does this mean?


==> sections/conclusion.tex <==
\subsection{Conclusion and Future Work}\label{sec:conclu}

%Fuzzing has played a critical role in many areas of software engineering, yet it remains largely unexplored from a mathematically rigorous perspective. In this paper, we provide a formal mathematical formulation of the fuzzing process and develop a theoretical evaluation framework for assessing fuzzer performance. Specifically, we model input generation and program feedback (output) as two separate Markov chains—one in the input space and the other in the output space. We propose a simulation algorithm that runs the input Markov chain and generates realizations of both the input and output chains, effectively mimicking the fuzzing process. We then perform output analysis on the output Markov chain, which leads to principled evaluation methods. We introduce a novel performance measure for the fuzzing process in both non-terminating and terminating regimes: the long-run and expected bug detection ratio (i.e., the ratio of inputs that lead to bugs among all inputs). To estimate this measure, we construct an empirical estimator by averaging the observed bug detection ratios over multiple runs. We define evaluation metrics for both the fuzzers (as the difference between the estimator and the true performance measure) and the duration of the fuzzing process. We also characterize the statistical properties of these estimators and metrics. Surprisingly, we find that a key factor in determining a fuzzer’s performance is the spectral gap—or equivalently, the relaxation time—of the output Markov chain. As a result, we present evaluation results for scenarios with and without prior knowledge of the software's bug detection ratio, as well as with and without access to the spectral information of the output Markov chain. Lastly, we numerically validate our results and evaluate multiple fuzzers on popular program benchmarks.

Fuzzing is critical to software security yet remains underexplored from a rigorous mathematical perspective. This paper formalizes the fuzzing process and introduces a unified theoretical–practical framework for evaluating fuzzers. We model input generation and program feedback as a Markov chain over inputs and a stochastic process over outputs, and propose a simulation algorithm that replicates fuzzing and unifies its objective. A new performance measure—the long-run and expected bug detection ratio, defined as the proportion of inputs triggering bugs—is introduced, along with an empirical estimator averaging observed ratios across runs. The resulting metrics quantify deviation from the true measure and dependence on fuzzing duration. We characterize their statistical properties and identify the spectral gap as a key performance determinant. Moving forward, designing new fuzzers that optimize (i.e., minimize) the spectral gap, formulated as an online optimization problem with the spectral gap as the objective, would be highly beneficial for practitioners. %\hl{add one sentence of how this spectral gap helps practioners/fuzzer design?} 
Extensive experiments with nine fuzzers across  benchmarks validate the framework. %under varying assumptions about bug detection ratios and spectral information.

Moving forward, developing efficient estimators for the unknown $\delta_R$ is a key direction. It also motivates designing rigorously principled fuzzers beyond heuristic methods. Finally, broadening the evaluation framework from mutation-based to grammar-based and white-box fuzzers remains an important goal.

%Moving forward, we highlight several promising directions. First, while our theoretical results apply to ergodic Markov chains, it would be valuable to extend the analysis to non-ergodic cases. Second, the current procedure for handling unknown \(\delta_R\) involves complex computations due to its general applicability to arbitrary Markov chains. This naturally motivates efforts to streamline the estimation of \(\delta_R\) for the specific Markov chains arising in our fuzz testing setting. Meanwhile, this new modeling framework calls for the design of rigorously effective fuzzers, moving beyond heuristic-based approaches; our findings could potentially help guide such developments. Lastly, although our evaluation framework is rigorous, it is currently limited to mutation-based fuzzers. Developing methods to capture the underlying stochastic dynamics of other types of fuzzers, e.g.\ grammar-based or white-box fuzzing, and constructing corresponding evaluation frameworks is an important direction.


\iffalse
\newpage

\begin{table*}[h]
\centering
\caption{Fuzzing progress across benchmarks and fuzzers.}\label{tab:fuzzing_progress_matrix}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{p{3.2cm}p{3cm}p{3cm}p{3cm}}
\toprule
\textbf{\makecell{Benchmark\(\arraybackslash\) \\ Fuzzer}} & \textbf{AFL} & \textbf{MOpt} & \textbf{Fairfuzz} \\
\midrule
libpng   & Setup complete; mutations under evaluation. & Coverage increasing steadily. & Execution stable; minor crashes observed. \\[3pt]
libjpeg  & Stable execution; no new crashes. & Corpus expansion in progress. & Coverage saturation detected. \\[3pt]
sqlite3  & Exploring rare branches. & Crash reproduction confirmed. & Corpus refinement ongoing. \\[3pt]
openssl  & Seed minimization in progress. & Stable runs; triaging crashes. & Coverage improving with deeper inputs. \\[3pt]
zlib     & Coverage plateau observed. & Stable; no new findings. & Extended runs planned. \\[3pt]
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[h]
\centering
\caption{Fuzzing progress across benchmarks and fuzzers.}\label{tab:fuzzing_progress_matrix}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{p{3.2cm}p{3cm}p{3cm}p{3cm}}
\toprule
\textbf{\makecell{Benchmark\(\arraybackslash\) \\ Fuzzer}} & \textbf{AFL++} & \textbf{libFuzzer} & \textbf{Honggfuzz} \\
\midrule
libpng   & Setup complete; mutations under evaluation. & Coverage increasing steadily. & Execution stable; minor crashes observed. \\[3pt]
libjpeg  & Stable execution; no new crashes. & Corpus expansion in progress. & Coverage saturation detected. \\[3pt]
sqlite3  & Exploring rare branches. & Crash reproduction confirmed. & Corpus refinement ongoing. \\[3pt]
openssl  & Seed minimization in progress. & Stable runs; triaging crashes. & Coverage improving with deeper inputs. \\[3pt]
zlib     & Coverage plateau observed. & Stable; no new findings. & Extended runs planned. \\[3pt]
\bottomrule
\end{tabular}
\end{table*}

\clearpage
\fi 

